To Copy, or not to Copy; That is a Critical Issue of the Output Softmax Layer in Neural Sequential Recommenders

Recent studies suggest that the existing neural models have difficulty handling repeated items in sequential recommendation tasks. However, our understanding of this difficulty is still limited. In this study, we substantially advance this field by identifying a major source of the problem: the single hidden state embedding and static item embeddings in the output softmax layer. Specifically, the similarity structure of the global item embeddings in the softmax layer sometimes forces the single hidden state embedding to be close to new items when copying is a better choice, while sometimes forcing the hidden state to be close to the items from the input inappropriately. To alleviate the problem, we adapt the recently-proposed softmax alternatives such as softmax-CPR to sequential recommendation tasks and demonstrate that the new softmax architectures unleash the capability of the neural encoder on learning when to copy and when to exclude the items from the input sequence. By only making some simple modifications on the output softmax layer for SASRec and GRU4Rec, softmax-CPR achieves consistent improvement in 12 datasets. With almost the same model size, our best method not only improves the average NDCG@10 of GRU4Rec in 5 datasets with duplicated items by 10% (4%-17% individually) but also improves 7 datasets without duplicated items by 24% (8%-39%)!

==> content/old_tables_fig.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.5\linewidth]{figs/Bridge_to_Algebra_(2008-2009)_fig.png}
  \caption{Math Exercise Recommendation}
  \label{fig:algebra}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.5\linewidth]{figs/Gowalla_fig.png}
  \caption{Location Recommendation}
  \label{fig:gowalla}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{figs/Steam_fig.png}
  \caption{Game Recommendation}
  \label{fig:steam}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{figs/Tmall-buy_fig.png}
  \caption{Shopping Recommendation}
  \label{fig:tmall}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{figs/Yoochoose-clicks_fig.png}
  \caption{E-commerical Clicking Recommendation}
  \label{fig:yoochoose}
\end{subfigure}
\caption{The probability of observing the item that has already been in the input sequence versus the sequence length. The blue curves are probability if the input sequence has already had duplicated items, while the orange curves indicate the probability when every item in the input sequence is unique.}
%Previous repeat. Previous unique. Sequence Length. Last Repeat Ratio. }
\label{fig:repeat_stats}
\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\scalebox{0.85}{
\begin{tabular}{cl|c|cc|ccccccccc|}
\multicolumn{1}{l}{}                   &                               & Model & Testing & Testing & \multicolumn{6}{c|}{Geometric Mean}                                                                                                   \\
 &                               & Size (M)                            & Time (s) & Time (s)                              & \multicolumn{3}{c}{7 datasets w/o dup.} & \multicolumn{3}{c}{5 datasets w/ dup.} & \multicolumn{3}{c|}{All 12 datasets} \\
                  &                               &                      &                               & NDCG                  & HIT                    & NDCG                  & HIT                   & NDCG             & HIT              \\
\multirow{9}{*}{\textbf{SAS}}          & Softmax                       & 5.34                                            & 22.43                                             & 4.79                  & 8.71                   & 31.60                 & 40.78                 & 10.75            & 16.88            \\
                                       & Softmax + Mi                    & 5.36                                            & 23.71                                             & 4.78                  & 8.79                   & 31.88                 & 40.87                 & 10.78            & 16.99            \\
                                       & Softmax + C                   & 5.35                                            & 28.53                                             & 5.55                  & 9.78                   & 33.59                 & 43.49                 & 12.01            & 18.53            \\
                                       & Softmax + CP                  & 5.36                                            & 29.13                                             & 5.64                  & 9.88                   & 33.78                 & 43.48                 & 12.15            & 18.65            \\
                                       & Softmax + CPR:100             & 5.37                                            & 34.43                                             & \textbf{5.72}         & 9.93                   & 34.04                 & 43.78                 & 12.28            & 18.75            \\
                                       & Softmax + CPR:100 + Mi        & 5.41                                            & 35.64                                             & 5.75                  & \textbf{10.11}         & 34.45                 & \textbf{44.06}        & \textbf{12.39}   & \textbf{19.00}   \\
                                       & Softmax + CPR:20,100,500 + Mi & 5.41                                            & 47.63                                             & 5.62                  & 9.80                   & \textbf{34.57}        & 43.93                 & 12.24            & 18.64            \\
                                       & MoS                           & 5.35                                            & 33.78                                             & 4.72                  & 8.71                   & 31.87                 & 41.10                 & 10.70            & 16.94            \\
                                       & Softmax w/o Duplication       & 5.34                                            & 22.61                                             & 5.40                  & 9.53                   & 10.22                 & 15.60                 & 7.09             & 11.77            \\ \hline
\multirow{9}{*}{\textbf{GRU4Rec}}      & Softmax                       & 5.42                                            & 31.24                                             & 4.85                  & 8.99                   & 31.20                 & 40.23                 & 10.77            & 17.09            \\
                                       & Softmax + Mi                  & 5.45                                            & 33.37                                             & 4.98                  & 9.14                   & 31.18                 & 40.19                 & 10.93            & 17.25            \\
                                       & Softmax + C                   & 5.42                                            & 37.84                                             & 5.75                  & 10.16                  & 33.55                 & 43.24                 & 12.24            & 18.90            \\
                                       & Softmax + CP                  & 5.43                                            & 38.45                                             & 5.76                  & 10.14                  & 33.80                 & 43.48                 & 12.29            & 18.93            \\
                                       & Softmax + CPR:100             & 5.44                                            & 43.18                                             & 6.02                  & 10.55                  & 34.27                 & 43.82                 & 12.68            & 19.42            \\
                                       & Softmax + CPR:100 + Mi        & 5.50                                            & 45.60                                             & \textbf{6.13}         & \textbf{10.69}         & 34.39                 & \textbf{43.83}        & \textbf{12.83}   & \textbf{19.57}   \\
                                       & Softmax + CPR:20,100,500 + Mi & 5.50                                            & 57.51                                             & 6.01                  & 10.44                  & \textbf{34.42}        & \textbf{43.83}        & 12.69            & 19.31            \\
                                       & MoS                           & 5.43                                            & 42.67                                             & 4.81                  & 8.91                   & 31.27                 & 40.15                 & 10.72            & 16.98            \\
                                       & Softmax w/o Duplication       & 5.42                                            & 31.00                                             & 5.52                  & 9.83                   & 10.06                 & 15.42                 & 7.14             & 11.92            \\ \hline
\multicolumn{1}{l}{\textbf{RepeatNet}} & Softmax                       &                                                 &                                                   & 5.63                  & 9.69                   & 33.43                 & 42.53                 & 12.08            & 18.27           
\end{tabular}
}
\caption{@10. We report the model size and time of testing the models on Amazon Book validation set. Mi is the multiple input hidden state enhancement; C is the context partition; R:20,100 is the reranker partition with $k_1=20$ and $k_2=100$; P is the pointer network (i.e., local decoder embedding). Please see \autoref{eq:logit_CPR} for the details of CPR.}
\label{tb:all_datasets}
%for getting the probabilities of next sequence in the validation set. }
\end{table*}

\begin{table*}[t!]
\centering
\scalebox{0.9}{
\begin{tabular}{cl|cccccccccc|}
\multicolumn{1}{l}{}                   &                               & \multicolumn{2}{c|}{Algebra}     & \multicolumn{2}{c|}{Gowalla}     & \multicolumn{2}{c|}{Steam}       & \multicolumn{2}{c|}{Tmall}       & \multicolumn{2}{c|}{Yoochoose}     \\
\multicolumn{1}{l}{}                   &                               & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}             \\ \hline
\multirow{9}{*}{\textbf{SAS}}          & Softmax                       & 85.66          & 90.42          & 29.28          & 40.39          & 15.67          & 20.28          & 22.44          & 26.60          & 35.74          & 57.28                          \\
                                       & Softmax + Mi                    & 85.68          & 89.72          & 29.72          & 40.72          & 15.60          & 20.10          & 22.64          & 26.80          & 36.62          & 57.93                      \\
                                       & Softmax + C                   & 86.25          & 91.15          & 32.23          & 45.15          & 16.32          & 21.13          & 25.29          & 30.36          & 37.26          & 58.93              \\
                                       & Softmax + CP                  & 85.60          & 89.75          & 32.88          & 45.68          & 16.31          & 21.05          & 25.58          & 30.50          & 37.43          & 59.02                    \\
                                       & Softmax + CPR:100             & 87.40          & 91.09          & 33.03          & 46.17          & 16.29          & 21.07          & 25.73          & 30.70          & 37.79          & 59.15                    \\
                                       & Softmax + CPR:100 + Mi        & 88.19          & \textbf{92.19} & 33.41          & 46.29          & \textbf{16.40}          & \textbf{21.32} & \textbf{25.74} & \textbf{30.58} & 39.03          & \textbf{59.69}  \\
                                       & Softmax + CPR:20,100,500 + Mi & \textbf{88.81} & 92.07          & \textbf{33.92} & \textbf{46.64} & 16.33 & 21.13          & 25.58          & 30.22          & \textbf{39.26} & 59.68             \\
                                       & MoS                           & 84.77          & 89.78          & 29.74          & 40.87          & 15.88          & 20.52          & 23.07          & 27.28          & 35.59          & 57.07                     \\
                                       & Softmax w/o Duplication       & 80.13          & 82.89          & 3.92           & 7.00           & 4.87           & 9.12           & 4.29           & 6.28           & 17.00          & 27.84           \\ \hline
\multirow{9}{*}{\textbf{GRU4Rec}}          & Softmax                       & 85.10          & 89.23          & 28.37          & 39.48          & 15.35          & 19.88          & 22.06          & 26.42          & 36.19          & 56.97            \\
                                       & Softmax + Mi                  & 84.68          & 89.01          & 27.99          & 39.06          & 15.69          & 20.26          & 21.76          & 26.05          & 36.39          & 57.15                   \\
                                       & Softmax + C                   & 85.86          & 89.75          & 32.23          & 45.18          & 16.29          & 21.04          & 25.18          & 30.25          & 37.46          & 58.54           \\
                                       & Softmax + CP                  & 86.24          & 91.06          & 32.48          & 45.43          & 16.32          & 21.06          & 25.45          & 30.36          & 37.90          & 58.76          \\
                                       & Softmax + CPR:100             & 88.56          & \textbf{92.35} & 33.01          & 46.08          & 16.36          & 21.15          & \textbf{25.77} & 30.34          & 38.35          & 59.15          \\
                                       & Softmax + CPR:100 + Mi        & 88.81          & 92.19          & \textbf{33.22} & \textbf{46.09} & \textbf{16.49} & \textbf{21.35} & 25.54          & 30.01          & \textbf{38.72} & \textbf{59.42} \\
                                       & Softmax + CPR:20,100,500 + Mi & \textbf{89.46} & 92.29          & 33.18          & 45.93          & 16.41          & 21.19          & 25.72          & \textbf{30.43} & 38.54          & 59.20          \\
                                       & MoS                           & 86.11          & 90.30          & 27.91          & 38.60          & 15.89          & 20.41          & 21.50          & 25.75          & 36.39          & 56.97          \\
                                       & Softmax w/o Duplication       & 79.06          & 81.67          & 3.93           & 7.05           & 4.65           & 8.72           & 4.24           & 6.32           & 16.80          & 27.44          \\ \hline
\multicolumn{1}{l}{\textbf{RepeatNet}} & Softmax                       & 77.72          & 82.19          & 33.83          & 45.88          & 16.28          & 20.90          & 25.67          & 30.17          & 38.00          & 58.53                

\end{tabular}
}
\caption{duplicated @10}
\label{tb:dup_dataset}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\scalebox{0.76}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{cl|cccccccccccccc|}
                   &                               & \multicolumn{6}{|c|}{Amazon}                                                                    & \multicolumn{4}{c|}{MovieLens}                                     & \multicolumn{2}{c|}{\multirow{2}{*}{Twitch}} & \multicolumn{2}{c|}{\multirow{2}{*}{Yelp}}  \\
\multicolumn{1}{l}{}                   &                               & \multicolumn{2}{c|}{Beauty}    & \multicolumn{2}{c|}{Book}      & \multicolumn{2}{c|}{Game}      & \multicolumn{2}{c|}{10m}         & \multicolumn{2}{c|}{1m}          & \multicolumn{2}{c|}{}                        & \multicolumn{2}{c|}{}                                             \\
\multicolumn{1}{l}{}                   &                               & NDCG          & \multicolumn{1}{c|}{HIT}           & NDCG          & \multicolumn{1}{c|}{HIT}           & NDCG          & \multicolumn{1}{c|}{HIT}           & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG                 & \multicolumn{1}{c|}{HIT}                  & NDCG                & \multicolumn{1}{c|}{HIT}\\ \hline
\multirow{9}{*}{\textbf{SAS}}          & Softmax                       & 1.18          & 2.06          & 3.30          & 5.81          & 3.93          & 7.67          & 15.72          & 26.67          & 17.19          & 29.85          & 8.41          & 15.51          & 1.66          & 3.36             \\
                                       & Softmax + Mi                    & 1.23          & 2.29          & 3.23          & 5.77          & 3.93          & 7.74          & 15.80          & 26.69          & 17.07          & 29.52          & 8.08          & 15.03          & 1.67          & 3.36         \\
                                       & Softmax + C                   & 1.33          & 2.32          & 3.83          & 6.46          & 4.47          & 8.31          & \textbf{19.12} & 31.13          & 21.06          & \textbf{35.15} & 9.14          & 16.39          & 1.94          & 3.82       \\
                                       & Softmax + CP                  & \textbf{1.36} & 2.31          & 3.94          & 6.71          & 4.49          & 8.41          & 18.62          & 30.51          & \textbf{21.08} & 34.97          & \textbf{9.45} & \textbf{16.93} & 2.04          & 3.91          \\
                                       & Softmax + CPR:100             & 1.34          & 2.29          & 4.15          & 6.89          & 4.49          & 8.29          & 19.32          & \textbf{31.32} & 20.41          & 34.27          & 9.11          & 15.94          & \textbf{2.22} & 4.24          \\
                                       & Softmax + CPR:100 + Mi        & \textbf{1.36} & \textbf{2.44} & \textbf{4.30} & \textbf{7.20} & \textbf{4.56} & \textbf{8.70} & 18.90          & 30.73          & 20.67          & 34.09          & 9.06          & 15.91          & 2.21          & 4.24          \\
                                       & Softmax + CPR:20,100,500 + Mi & 1.34          & 2.35          & 3.93          & 6.60          & 4.47          & 8.35          & 19.19          & 30.93          & 20.70          & 34.19          & 8.58          & 14.88          & 2.20          & \textbf{4.27}  \\
                                       & MoS                           & 1.10          & 2.15          & 3.24          & 5.75          & 3.88          & 7.49          & 15.88          & 26.82          & 17.15          & 29.59          & 8.17          & 15.19          & 1.69          & 3.42            \\
                                       & Softmax w/o Duplication       & 1.31          & 2.26          & 3.73          & 6.27          & 4.44          & 8.39          & 18.35          & 30.19          & 20.06          & 33.81          & 9.01          & 16.13          & 1.85          & 3.64          \\ \hline
\multirow{9}{*}{\textbf{GRU4Rec}}          & Softmax                       & 1.43          & 2.67          & 3.09          & 5.70          & 4.45          & 8.64          & 14.19          & 24.17          & 16.05          & 28.03          & 8.36          & 15.55          & 1.68          & 3.42 \\
                                       & Softmax + Mi                  & 1.47          & 2.69          & 3.30          & 5.92          & 4.58          & 8.79          & 14.58          & 25.04          & 16.55          & 28.94          & 8.03          & 14.98          & 1.76          & 3.52            \\
                                       & Softmax + C                   & 1.59          & 2.88          & 3.97          & 6.66          & 4.95          & 9.36          & 17.78          & 29.24          & 20.01          & 32.86          & 9.25          & 16.50          & 2.02          & 3.92           \\
                                       & Softmax + CP                  & 1.61          & 2.94          & 4.07          & 6.83          & \textbf{5.10} & 9.41          & 17.46          & 28.64          & 19.63          & 32.91          & 9.14          & 16.09          & 2.00          & 3.85           \\
                                       & Softmax + CPR:100             & \textbf{1.78} & \textbf{3.22} & 4.28          & 7.06          & 5.05          & \textbf{9.49} & 17.78          & 29.01          & 20.35          & 33.73          & 9.04          & 15.82          & 2.27          & 4.35           \\
                                       & Softmax + CPR:100 + Mi        & 1.72          & 3.15          & 4.42          & \textbf{7.23} & 5.07          & 9.43          & \textbf{18.09} & \textbf{29.43} & \textbf{21.00} & \textbf{34.52} & \textbf{9.32} & \textbf{16.20} & \textbf{2.37} & \textbf{4.51}  \\
                                       & Softmax + CPR:20,100,500 + Mi & 1.73          & 3.11          & \textbf{4.37} & 7.14          & 5.02          & 9.33          & 17.87          & 29.09          & 20.44          & 33.63          & 8.80          & 15.20          & 2.31          & 4.39          \\
                                       & MoS                           & 1.46          & 2.73          & 3.15          & 5.76          & 4.06          & 8.00          & 14.40          & 24.50          & 16.14          & 28.06          & 7.90          & 14.69          & 1.73          & 3.50           \\
                                       & Softmax w/o Duplication       & 1.60          & 2.91          & 3.71          & 6.26          & 4.83          & 9.09          & 16.85          & 27.68          & 18.54          & 31.72          & 8.94          & 16.03          & 1.94          & 3.80         \\ \hline
\multicolumn{1}{l}{\textbf{RepeatNet}} & Softmax                       & 1.75          & 2.88          & 3.94          & 6.36          & 4.47          & 8.36          & 18.09          & 29.20          & 18.71          & 31.08          & 8.52          & 14.91          & 2.02          & 3.88            

\end{tabular}
}
\caption{@10. percentage. best within each section is highlighted. test datasets}
\label{tb:nodup_dataset}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\scalebox{0.73}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{cl|cccccccccccccccc}
                   &                               & \multicolumn{6}{|c|}{Amazon}                                                                    & \multicolumn{4}{c|}{MovieLens}                                     & \multicolumn{2}{c|}{\multirow{2}{*}{Twitch}} & \multicolumn{2}{c|}{\multirow{2}{*}{Yelp}} & \multicolumn{2}{c|}{\multirow{2}{*}{Gmean   (Unique)}} \\
\multicolumn{1}{l}{}                   &                               & \multicolumn{2}{c|}{Beauty}    & \multicolumn{2}{c|}{Book}      & \multicolumn{2}{c|}{Game}      & \multicolumn{2}{c|}{10m}         & \multicolumn{2}{c|}{1m}          & \multicolumn{2}{c|}{}                        & \multicolumn{2}{c|}{}                      & \multicolumn{2}{c|}{}                                        \\
\multicolumn{1}{l}{}                   &                               & NDCG          & \multicolumn{1}{c|}{HIT}           & NDCG          & \multicolumn{1}{c|}{HIT}           & NDCG          & \multicolumn{1}{c|}{HIT}           & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG                 & \multicolumn{1}{c|}{HIT}                  & NDCG                & \multicolumn{1}{c|}{HIT}                 & NDCG                         & \multicolumn{1}{c|}{HIT}                          \\ \hline
\multirow{9}{*}{\textbf{SAS}}          & Softmax                       & 1.18          & 2.06          & 3.30          & 5.81          & 3.93          & 7.67          & 15.72          & 26.67          & 17.19          & 29.85          & 8.41          & 15.51          & 1.66          & 3.36          & 4.79          & 8.71           \\
                                       & Softmax + Mi                    & 1.23          & 2.29          & 3.23          & 5.77          & 3.93          & 7.74          & 15.80          & 26.69          & 17.07          & 29.52          & 8.08          & 15.03          & 1.67          & 3.36          & 4.78          & 8.79           \\
                                       & Softmax + C                   & 1.33          & 2.32          & 3.83          & 6.46          & 4.47          & 8.31          & \textbf{19.12} & 31.13          & 21.06          & \textbf{35.15} & 9.14          & 16.39          & 1.94          & 3.82          & 5.55          & 9.78           \\
                                       & Softmax + CP                  & \textbf{1.36} & 2.31          & 3.94          & 6.71          & 4.49          & 8.41          & 18.62          & 30.51          & \textbf{21.08} & 34.97          & \textbf{9.45} & \textbf{16.93} & 2.04          & 3.91          & 5.64          & 9.88           \\
                                       & Softmax + CPR:100             & 1.34          & 2.29          & 4.15          & 6.89          & 4.49          & 8.29          & 19.32          & \textbf{31.32} & 20.41          & 34.27          & 9.11          & 15.94          & \textbf{2.22} & 4.24          & \textbf{5.72} & 9.93           \\
                                       & Softmax + CPR:100 + Mi        & \textbf{1.36} & \textbf{2.44} & \textbf{4.30} & \textbf{7.20} & \textbf{4.56} & \textbf{8.70} & 18.90          & 30.73          & 20.67          & 34.09          & 9.06          & 15.91          & 2.21          & 4.24          & 5.75          & \textbf{10.11} \\
                                       & Softmax + CPR:20,100,500 + Mi & 1.34          & 2.35          & 3.93          & 6.60          & 4.47          & 8.35          & 19.19          & 30.93          & 20.70          & 34.19          & 8.58          & 14.88          & 2.20          & \textbf{4.27} & 5.62          & 9.80           \\
                                       & MoS                           & 1.10          & 2.15          & 3.24          & 5.75          & 3.88          & 7.49          & 15.88          & 26.82          & 17.15          & 29.59          & 8.17          & 15.19          & 1.69          & 3.42          & 4.72          & 8.71           \\
                                       & Softmax w/o Duplication       & 1.31          & 2.26          & 3.73          & 6.27          & 4.44          & 8.39          & 18.35          & 30.19          & 20.06          & 33.81          & 9.01          & 16.13          & 1.85          & 3.64          & 5.40          & 9.53           \\ \hline
\multirow{9}{*}{\textbf{GRU4Rec}}          & Softmax                       & 1.43          & 2.67          & 3.09          & 5.70          & 4.45          & 8.64          & 14.19          & 24.17          & 16.05          & 28.03          & 8.36          & 15.55          & 1.68          & 3.42          & 4.85          & 8.99           \\
                                       & Softmax + Mi                  & 1.47          & 2.69          & 3.30          & 5.92          & 4.58          & 8.79          & 14.58          & 25.04          & 16.55          & 28.94          & 8.03          & 14.98          & 1.76          & 3.52          & 4.98          & 9.14           \\
                                       & Softmax + C                   & 1.59          & 2.88          & 3.97          & 6.66          & 4.95          & 9.36          & 17.78          & 29.24          & 20.01          & 32.86          & 9.25          & 16.50          & 2.02          & 3.92          & 5.75          & 10.16          \\
                                       & Softmax + CP                  & 1.61          & 2.94          & 4.07          & 6.83          & \textbf{5.10} & 9.41          & 17.46          & 28.64          & 19.63          & 32.91          & 9.14          & 16.09          & 2.00          & 3.85          & 5.76          & 10.14          \\
                                       & Softmax + CPR:100             & \textbf{1.78} & \textbf{3.22} & 4.28          & 7.06          & 5.05          & \textbf{9.49} & 17.78          & 29.01          & 20.35          & 33.73          & 9.04          & 15.82          & 2.27          & 4.35          & 6.02          & 10.55          \\
                                       & Softmax + CPR:100 + Mi        & 1.72          & 3.15          & 4.42          & \textbf{7.23} & 5.07          & 9.43          & \textbf{18.09} & \textbf{29.43} & \textbf{21.00} & \textbf{34.52} & \textbf{9.32} & \textbf{16.20} & \textbf{2.37} & \textbf{4.51} & \textbf{6.13} & \textbf{10.69} \\
                                       & Softmax + CPR:20,100,500 + Mi & 1.73          & 3.11          & \textbf{4.37} & 7.14          & 5.02          & 9.33          & 17.87          & 29.09          & 20.44          & 33.63          & 8.80          & 15.20          & 2.31          & 4.39          & 6.01          & 10.44          \\
                                       & MoS                           & 1.46          & 2.73          & 3.15          & 5.76          & 4.06          & 8.00          & 14.40          & 24.50          & 16.14          & 28.06          & 7.90          & 14.69          & 1.73          & 3.50          & 4.81          & 8.91           \\
                                       & Softmax w/o Duplication       & 1.60          & 2.91          & 3.71          & 6.26          & 4.83          & 9.09          & 16.85          & 27.68          & 18.54          & 31.72          & 8.94          & 16.03          & 1.94          & 3.80          & 5.52          & 9.83           \\ \hline
\multicolumn{1}{l}{\textbf{RepeatNet}} & Softmax                       & 1.75          & 2.88          & 3.94          & 6.36          & 4.47          & 8.36          & 18.09          & 29.20          & 18.71          & 31.08          & 8.52          & 14.91          & 2.02          & 3.88          & 5.63          & 9.69          

\end{tabular}
}
\caption{@10. percentage. best within each section is highlighted. test datasets}
\end{table*}


\begin{table*}[t!]
\centering
\scalebox{0.73}{
\begin{tabular}{cl|cccccccccccccc}
\multicolumn{1}{l}{}                   &                               & \multicolumn{2}{c|}{Algebra}     & \multicolumn{2}{c|}{Gowalla}     & \multicolumn{2}{c|}{Steam}       & \multicolumn{2}{c|}{Tmall}       & \multicolumn{2}{c|}{Yoochoose}   & \multicolumn{2}{c|}{Gmean (Duplicated)} & \multicolumn{2}{c|}{Gmean (All)} \\
\multicolumn{1}{l}{}                   &                               & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG           & \multicolumn{1}{c|}{HIT}            & NDCG               & \multicolumn{1}{c|}{HIT}               & NDCG           & \multicolumn{1}{c|}{HIT}            \\ \hline
\multirow{9}{*}{\textbf{SAS}}          & Softmax                       & 85.66          & 90.42          & 29.28          & 40.39          & 15.67          & 20.28          & 22.44          & 26.60          & 35.74          & 57.28          & 31.60          & 40.78          & 10.75          & 16.88          \\
                                       & Softmax + Mi                    & 85.68          & 89.72          & 29.72          & 40.72          & 15.60          & 20.10          & 22.64          & 26.80          & 36.62          & 57.93          & 31.88          & 40.87          & 10.78          & 16.99          \\
                                       & Softmax + C                   & 86.25          & 91.15          & 32.23          & 45.15          & 16.32          & 21.13          & 25.29          & 30.36          & 37.26          & 58.93          & 33.59          & 43.49          & 12.01          & 18.53          \\
                                       & Softmax + CP                  & 85.60          & 89.75          & 32.88          & 45.68          & 16.31          & 21.05          & 25.58          & 30.50          & 37.43          & 59.02          & 33.78          & 43.48          & 12.15          & 18.65          \\
                                       & Softmax + CPR:100             & 87.40          & 91.09          & 33.03          & 46.17          & 16.29          & 21.07          & 25.73          & 30.70          & 37.79          & 59.15          & 34.04          & 43.78          & 12.28          & 18.75          \\
                                       & Softmax + CPR:100 + Mi        & 88.19          & \textbf{92.19} & 33.41          & 46.29          & \textbf{16.40}          & \textbf{21.32} & \textbf{25.74} & \textbf{30.58} & 39.03          & \textbf{59.69} & 34.45          & \textbf{44.06} & \textbf{12.39} & \textbf{19.00} \\
                                       & Softmax + CPR:20,100,500 + Mi & \textbf{88.81} & 92.07          & \textbf{33.92} & \textbf{46.64} & 16.33 & 21.13          & 25.58          & 30.22          & \textbf{39.26} & 59.68          & \textbf{34.57} & 43.93          & 12.24          & 18.64          \\
                                       & MoS                           & 84.77          & 89.78          & 29.74          & 40.87          & 15.88          & 20.52          & 23.07          & 27.28          & 35.59          & 57.07          & 31.87          & 41.10          & 10.70          & 16.94          \\
                                       & Softmax w/o Duplication       & 80.13          & 82.89          & 3.92           & 7.00           & 4.87           & 9.12           & 4.29           & 6.28           & 17.00          & 27.84          & 10.22          & 15.60          & 7.09           & 11.77          \\ \hline
\multirow{9}{*}{\textbf{GRU4Rec}}          & Softmax                       & 85.10          & 89.23          & 28.37          & 39.48          & 15.35          & 19.88          & 22.06          & 26.42          & 36.19          & 56.97          & 31.20          & 40.23          & 10.77          & 17.09          \\
                                       & Softmax + Mi                  & 84.68          & 89.01          & 27.99          & 39.06          & 15.69          & 20.26          & 21.76          & 26.05          & 36.39          & 57.15          & 31.18          & 40.19          & 10.93          & 17.25          \\
                                       & Softmax + C                   & 85.86          & 89.75          & 32.23          & 45.18          & 16.29          & 21.04          & 25.18          & 30.25          & 37.46          & 58.54          & 33.55          & 43.24          & 12.24          & 18.90          \\
                                       & Softmax + CP                  & 86.24          & 91.06          & 32.48          & 45.43          & 16.32          & 21.06          & 25.45          & 30.36          & 37.90          & 58.76          & 33.80          & 43.48          & 12.29          & 18.93          \\
                                       & Softmax + CPR:100             & 88.56          & \textbf{92.35} & 33.01          & 46.08          & 16.36          & 21.15          & \textbf{25.77} & 30.34          & 38.35          & 59.15          & 34.27          & 43.82          & 12.68          & 19.42          \\
                                       & Softmax + CPR:100 + Mi        & 88.81          & 92.19          & \textbf{33.22} & \textbf{46.09} & \textbf{16.49} & \textbf{21.35} & 25.54          & 30.01          & \textbf{38.72} & \textbf{59.42} & 34.39          & \textbf{43.83} & \textbf{12.83} & \textbf{19.57} \\
                                       & Softmax + CPR:20,100,500 + Mi & \textbf{89.46} & 92.29          & 33.18          & 45.93          & 16.41          & 21.19          & 25.72          & \textbf{30.43} & 38.54          & 59.20          & \textbf{34.42} & \textbf{43.83} & 12.69          & 19.31          \\
                                       & MoS                           & 86.11          & 90.30          & 27.91          & 38.60          & 15.89          & 20.41          & 21.50          & 25.75          & 36.39          & 56.97          & 31.27          & 40.15          & 10.72          & 16.98          \\
                                       & Softmax w/o Duplication       & 79.06          & 81.67          & 3.93           & 7.05           & 4.65           & 8.72           & 4.24           & 6.32           & 16.80          & 27.44          & 10.06          & 15.42          & 7.14           & 11.92          \\ \hline
\multicolumn{1}{l}{\textbf{RepeatNet}} & Softmax                       & 77.72          & 82.19          & 33.83          & 45.88          & 16.28          & 20.90          & 25.67          & 30.17          & 38.00          & 58.53          & 33.43          & 42.53          & 12.08          & 18.27         

\end{tabular}
}
\caption{duplicated @10}
\end{table*}
